A Dataset of German Legal Documents for Named Entity Recognition

We describe a dataset developed for Named Entity Recognition in German federal court decisions. It consists of approx. 67,000 sentences with over 2 million tokens. The resource contains 54,000 manually annotated entities, mapped to 19 fine-grained semantic classes: person, judge, lawyer, country, city, street, landscape, organization, company, institution, court, brand, law, ordinance, European legal norm, regulation, contract, court decision, and legal literature. The legal documents were, furthermore, automatically annotated with more than 35,000 TimeML-based time expressions. The dataset, which is available under a CC-BY 4.0 license in the CoNNL-2002 format, was developed for training an NER service for German legal documents in the EU project Lynx.

==> tables/fine_coarse.tex <==
\begin{table}[ht]
\centering
\footnotesize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{{\textbf{\#}}} & \multicolumn{2}{c}{\textbf{coarse-grained}}                    & \multicolumn{1}{|c|}{{\textbf{\#}}} & \multicolumn{2}{c|}{\textbf{fine-grained}} \\
\hline
\textbf{1}                                 & \textbf{PER}                               &  person                                  &  \textbf{1}                       & \textbf{PER}                      & person                             \\

     &  &        &  \textbf{2}                       & \textbf{RR}                       & judge                              \\

                                 &                                &                                    &  \textbf{3}                       & \textbf{AN}                       & lawyer                              \\ %\cline{3-3} \cline{6-6} 
\hline
\textbf{2}                                 & \textbf{LOC}                               & location                                   & {\textbf{4}}                       & \textbf{LD}                       & country                               \\
                                 &                                &                                    &  \textbf{5}                       & \textbf{ST}                       & city                               \\

                                 &                                &                                    &  \textbf{6}                       & \textbf{STR}                      & street                              \\

     &  &              &\textbf{7}                       & \textbf{LDS}                      & landscape                           \\ %\cline{3-3} \cline{6-6}
\hline
\textbf{3}                                 & \textbf{ORG}                               &  organization                                  &{\textbf{8}}                       & \textbf{ORG}                      & organization                       \\

{ }                                 &                                &                                    & {\textbf{9}}                       & \textbf{UN}                       & company                          \\

{ }                                 &                                &                                    & {\textbf{10}}                      & \textbf{INN}                      & institution                        \\
{ }                                 &                                &                                    & {\textbf{11}}                      & \textbf{GRT}                      & court                             \\

     &  & & {\textbf{12}}                      & \textbf{MRK}                      & brand                               \\ %\cline{3-3} \cline{6-6}
\hline
{\textbf{4} }                                 & \textbf{NRM}                               &          legal norm                          & {\textbf{13}}                      & \textbf{GS}                       & law                              \\ 
{ }                                 &                                &                                    & {\textbf{14}}                      & \textbf{VO}                       & ordinance                         \\
     &  &      & {\textbf{15}}                      & \textbf{EUN}                      & EU norm                            \\ %\cline{3-3}\cline{6-6}
\hline
{\textbf{5} }                                 & \textbf{REG}                               &          case-by-case                          & {\textbf{16}}                      & \textbf{VS}                       & regulation                         \\
                                 &                                &  regulation                                  & {\textbf{17}}                      & \textbf{VT}                       & contract                             \\ %\cline{3-3} \cline{6-6}
\hline
{\textbf{6}}                       & \textbf{RS}                                           & desicion                          & {\textbf{18}}                      & \textbf{RS}             & desicion  \\  %\cline{3-3} \cline{6-6}   
\hline
{\textbf{7}}                       & \textbf{LIT}                                           & literature                          & {\textbf{19}}                      & \textbf{LIT}                      & literature \\
\hline
\end{tabular}
\caption{VLLT BRAUCHT MAN DIESE TABELLE NICHT}
\label{classes}
\end{table}

==> tables/stat_cg.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|r|l|}
\hline
\multicolumn{3}{|c|}{\textbf{Coarse-grained classes}} & \multicolumn{1}{c|}{\textbf{\#}} & \multicolumn{1}{c|}{\textbf{\%}} \\ \hline \hline
1          & PER          & Person                    & 3,377                           & 6.30                             \\ \hline
2          & LOC          & Location                  & 2,468                           & 4.60                             \\ \hline
3          & ORG          & Organization              & 7,915                           & 14.76                            \\ \hline
4          & NRM          & Legal norm                & 20,816                          & 38.81                            \\ \hline
5          & REG          & Case-by-case              & 3,470                           & 6.47                             \\ \hline
6          & RS           & Court decision            & 12,580                          & 23.46                            \\ \hline
7          & LIT          & Legal literature          & 3,006                           & 5.60                             \\ \hline \hline
\multicolumn{3}{|l|}{\textbf{Total}}                  & \textbf{53,632}                 & \textbf{100}                     \\ \hline
\end{tabular}
\caption{Distribution of coarse-grained classes in dataset}
\label{stat_cg}
\end{table}

==> tables/stat_fg.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|l|l|l|r|l|}
\hline
\multicolumn{3}{|c|}{\textbf{Fine-grained classes}} & \multicolumn{1}{c|}{\textbf{\#}} & \multicolumn{1}{c|}{\textbf{\%}} \\ \hline \hline
1         & PER        & Person                     & 1,747                           & 3.26                             \\ \hline
2         & RR         & Judge                      & 1,519                           & 2.83                             \\ \hline
3         & AN         & Lawyer                     & 111                              & 0.21                             \\ \hline \hline
4         & LD         & Country                    & 1,429                           & 2.66                             \\ \hline
5         & ST         & City                       & 705                              & 1.31                             \\ \hline
6         & STR        & Street                     & 136                              & 0.25                             \\ \hline
7         & LDS        & Landscape                  & 198                              & 0.37                             \\ \hline \hline
8         & ORG        & Organization               & 1,166                           & 2.17                             \\ \hline
9         & UN         & Company                    & 1,058                           & 1.97                             \\ \hline
10        & INN        & Institution                & 2,196                           & 4.09                             \\ \hline
11        & GRT        & Court                      & 3,212                           & 5.99                             \\ \hline
12        & MRK        & Brand                      & 283                              & 0.53                             \\ \hline \hline
13        & GS         & Law                        & 18,520                          & 34.53                            \\ \hline
14        & VO         & Ordinance                  & 797                              & 1.49                             \\ \hline
15        & EUN        & European legal norm        & 1,499                           & 2.79                             \\ \hline \hline
16        & VS         & Regulation                 & 607                              & 1.13                             \\ \hline
17        & VT         & Contract                   & 2,863                           & 5.34                             \\ \hline \hline
18        & RS         & Court decision             & 12,580                          & 23.46                            \\ \hline \hline
19        & LIT        & Legal literature           & 3,006                           & 5.60                             \\ \hline \hline
\multicolumn{3}{|l|}{\textbf{Total}}                & \textbf{53,632}                 & \textbf{100}                     \\ \hline
\end{tabular}
\caption{Distribution of fine-grained classes in dataset}
\label{stat_fg}
\end{table}
